Model-Based Monitoring and State Estimation for Digital Twins: The Kalman Filter

A digital twin (DT) monitors states of the physical twin (PT) counterpart and provides a number of benefits such as advanced visualizations, fault detection capabilities, and reduced maintenance cost. It is the ability to be able to detect the states inside the DT that enable such benefits. In order to estimate the desired states of a PT, we propose the use of a Kalman Filter (KF). In this tutorial, we provide an introduction and detailed derivation of the KF. We demonstrate the use of KF to monitor and anomaly detection through an incubator system. Our experimental result shows that KF successfully can detect the anomaly during monitoring.

==> author.tex <==
\section*{Author Biographies}

\textbf{\uppercase{Hao Feng}} is a PhD Student at Aarhus University specializing in the fundamental techniques that make up Digital Twins, including monitoring. His PhD combines software and robotics.

\textbf{\uppercase{CLÁUDIO GOMES}} is a postdoc researcher at Aarhus University (Denmark). He received his PhD at the University of Antwerp, for his work on the foundations of co-simulation, one of the fundamental techniques enabling the DT. His web address is \url{ http://pure.au.dk/portal/en/claudio.gomes@eng.au.dk}.

% \textbf{\uppercase{Alexandros Iosifidis}} is an associate professor at Aarhus University.  His research interests include topics of neural networks, deep/representation learning and statistical machine learning.

\textbf{\uppercase{Alexandros Iosifidis}} is an associate professor at Aarhus University.  His research interests include topics of neural networks, deep/representation learning and statistical machine learning.


\textbf{\uppercase{Peter Gorm Larsen}} is a professor at Aarhus University.
He has been involved with >40 research projects and he currently leads the AU DIGIT Centre of Digitalisation, Big Data and Data Analytics, the AU Centre for Digital Twins, as well as the research group for Cyber-Physical Systems.
He has published more than 200 articles and three books on modelling of cyber-physical systems and digital twins.

